Studying and Benchmarking Large Language Models For Log Level Suggestion

Large Language Models (LLMs) have become a focal point of research across various domains, including software engineering, where their capabilities are increasingly leveraged. Recent studies have explored the integration of LLMs into software development tools and frameworks, revealing their potential to enhance performance in text and code-related tasks. Log level is a key part of a logging statement that allows software developers control the information recorded during system runtime. Given that log messages often mix natural language with code-like variables, LLMs' language translation abilities could be applied to determine the suitable verbosity level for logging statements. In this paper, we undertake a detailed empirical analysis to investigate the impact of characteristics and learning paradigms on the performance of 12 open-source LLMs in log level suggestion. We opted for open-source models because they enable us to utilize in-house code while effectively protecting sensitive information and maintaining data security. We examine several prompting strategies, including Zero-shot, Few-shot, and fine-tuning techniques, across different LLMs to identify the most effective combinations for accurate log level suggestions. Our research is supported by experiments conducted on 9 large-scale Java systems. The results indicate that although smaller LLMs can perform effectively with appropriate instruction and suitable techniques, there is still considerable potential for improvement in their ability to suggest log levels.

==> textfiles/discussion.tex <==
How often is getting N/A in models?
Are the N/A more prevalent in Llama or CodeLlama

Are N/A more prevalent in Finetuned models?

Does stratified fine-tuning dataset affecting the results distribution?

Is there a preference in log levels based on different LLMs?

How many logs are correctly predicted in all LLMs?

For Fill-Mask LLMs, the maximum number of correct predictions across all LLMs is 56, yet the highest number of correct prediction achieved is 51.

For Generative LLMs, max number is 28, but highest is 26. 

If we use generative LLMs, regardless if it is NLP or Code-based model type, we find that the distribution is always either all correct, or all wrong.
If use Fill-Mask, it is always (except for graphcode bert) one of them is always correct, the percentage of all correct is always the lowest.
